GW170817: Implications for the Stochastic Gravitational-Wave Background from Compact Binary Coalescences

The LIGO Scientific and Virgo Collaborations have announced the first detection of gravitational waves from the coalescence of two neutron stars. The merger rate of binary neutron stars estimated from this event suggests that distant, unresolvable binary neutron stars create a significant astrophysical stochastic gravitational-wave background. The binary neutron star background will add to the background from binary black holes, increasing the amplitude of the total astrophysical background relative to previous expectations. In the Advanced LIGO-Virgo frequency band most sensitive to stochastic backgrounds (near 25 Hz), we predict a total astrophysical background with amplitude $\Omega_{\rm GW} (f=25 \text{Hz}) = 1.8_{-1.3}^{+2.7} \times 10^{-9}$ with $90\%$ confidence, compared with $\Omega_{\rm GW} (f=25 \text{Hz}) = 1.1_{-0.7}^{+1.2} \times 10^{-9}$ from binary black holes alone. Assuming the most probable rate for compact binary mergers, we find that the total background may be detectable with a signal-to-noise-ratio of 3 after 40 months of total observation time, based on the expected timeline for Advanced LIGO and Virgo to reach their design sensitivity.

==> GW170817_ Implications for the Stochastic Gravitational-Wave Background from Compact Binary Coalescences/LVC_Aug2017.tex <==
%%\documentclass[aps,prd,superscriptaddress,altaffilletter]{revtex4-1}
%\documentclass[aps,prd,superscriptaddress]{revtex4-1}
%\begin{document}

%\title{LSC August 2017 and Virgo August 2017 author list---LIGO-M1700231}

%\begin{abstract}
%This is the LSC August 2017 and Virgo August 2017 author list---LIGO-M1700231.
%\end{abstract}

% added Joe Romano (opt-in status)

\author{%
B.~P.~Abbott,$^{1}$  %benjamin.abbott
R.~Abbott,$^{1}$  %rich.abbott
T.~D.~Abbott,$^{2}$  %thomas.abbott
F.~Acernese,$^{3,4}$ %fausto.acernese
K.~Ackley,$^{5,6}$  %kendall.ackley
C.~Adams,$^{7}$  %carl.adams
T.~Adams,$^{8}$ %thomas.adams
P.~Addesso,$^{9}$  %paolo.addesso
R.~X.~Adhikari,$^{1}$  %rana.adhikari
V.~B.~Adya,$^{10}$  %vaishali.adya
C.~Affeldt,$^{10}$  %christoph.affeldt
M.~Afrough,$^{11}$  %mohammad.afrough
B.~Agarwal,$^{12}$  %bhanu.agarwal
M.~Agathos,$^{13}$  %michalis.agathos
K.~Agatsuma,$^{14}$ %kazuhiro.agatsuma
N.~Aggarwal,$^{15}$  %nancy.aggarwal
O.~D.~Aguiar,$^{16}$  %odylio.aguiar
L.~Aiello,$^{17,18}$ %lorenzo.aiello
A.~Ain,$^{19}$  %anirban.ain
P.~Ajith,$^{20}$  %ajith.parameswaran
B.~Allen,$^{10,21,22}$  %bruce.allen
G.~Allen,$^{12}$  %gabrielle.allen
A.~Allocca,$^{23,24}$ %annalisa.allocca
P.~A.~Altin,$^{25}$  %paul.altin
A.~Amato,$^{26}$ %alex.amato
A.~Ananyeva,$^{1}$  %alena.ananyeva
S.~B.~Anderson,$^{1}$  %stuart.anderson
W.~G.~Anderson,$^{21}$  %warren.anderson
S.~V.~Angelova,$^{27}$  %svetoslava.angelova
S.~Antier,$^{28}$ %sarah.antier
S.~Appert,$^{1}$  %stephen.appert
K.~Arai,$^{1}$  %koji.arai
M.~C.~Araya,$^{1}$  %melody.araya
J.~S.~Areeda,$^{29}$  %joseph.areeda
N.~Arnaud,$^{28,30}$ %nicolas.arnaud
K.~G.~Arun,$^{31}$  %kg.arun
S.~Ascenzi,$^{32,33}$ %stefano.ascenzi
G.~Ashton,$^{10}$  %gregory.ashton
M.~Ast,$^{34}$  %melanie.meinders
S.~M.~Aston,$^{7}$  %stuart.aston
P.~Astone,$^{35}$ %pia.astone
D.~V.~Atallah,$^{36}$  %dany.atallah
P.~Aufmuth,$^{22}$  %peter.aufmuth
C.~Aulbert,$^{10}$  %carsten.aulbert
K.~AultONeal,$^{37}$  %kellie.aultoneal
C.~Austin,$^{2}$	%corey.austin
A.~Avila-Alvarez,$^{29}$  %adrian.avila-alvarez
S.~Babak,$^{38}$  %stanislav.babak
P.~Bacon,$^{39}$ %philippe.bacon
M.~K.~M.~Bader,$^{14}$ %maria.bader
S.~Bae,$^{40}$  %sangwook.bae
P.~T.~Baker,$^{41}$  %paul.baker
F.~Baldaccini,$^{42,43}$ %francesca.baldaccini
G.~Ballardin,$^{30}$ %giulio.ballardin
S.~W.~Ballmer,$^{44}$  %stefan.ballmer
S.~Banagiri,$^{45}$  %sharan.banagiri
J.~C.~Barayoga,$^{1}$  %juan.barayoga
S.~E.~Barclay,$^{46}$  %sheena.barclay
B.~C.~Barish,$^{1}$  %barry.barish
D.~Barker,$^{47}$  %david.barker
K.~Barkett,$^{48}$  %kevin.barkett
F.~Barone,$^{3,4}$ %fabrizio.barone
B.~Barr,$^{46}$  %bryan.barr
L.~Barsotti,$^{15}$  %lisa.barsotti
M.~Barsuglia,$^{39}$ %matteo.barsuglia
D.~Barta,$^{49}$ %daniel.barta
J.~Bartlett,$^{47}$  %jeffrey.bartlett
I.~Bartos,$^{50,5}$  %imre.bartos
R.~Bassiri,$^{51}$  %riccardo.bassiri
A.~Basti,$^{23,24}$ %andrea.basti
J.~C.~Batch,$^{47}$  %james.batch
M.~Bawaj,$^{52,43}$ %mateusz.bawaj
J.~C.~Bayley,$^{46}$  %joseph.bayley
M.~Bazzan,$^{53,54}$ %marco.bazzan
B.~B\'ecsy,$^{55}$  %bence.becsy
C.~Beer,$^{10}$  %christian.beer
M.~Bejger,$^{56}$ %michal.bejger
I.~Belahcene,$^{28}$ %imene.belahcene
A.~S.~Bell,$^{46}$  %angus.bell
B.~K.~Berger,$^{1}$  %beverly.berger
G.~Bergmann,$^{10}$  %gerald.bergmann
J.~J.~Bero,$^{57}$  %john.bero
C.~P.~L.~Berry,$^{58}$  %christopher.berry
D.~Bersanetti,$^{59}$ %diego.bersanetti
A.~Bertolini,$^{14}$ %alessandro.bertolini
J.~Betzwieser,$^{7}$  %joseph.betzwieser
S.~Bhagwat,$^{44}$  %swetha.bhagwat
R.~Bhandare,$^{60}$  %rohan.bhandare
I.~A.~Bilenko,$^{61}$  %igor.bilenko
G.~Billingsley,$^{1}$  %garilynn.billingsley
C.~R.~Billman,$^{5}$  %chris.billman
J.~Birch,$^{7}$  %jeremy.birch
R.~Birney,$^{62}$  %ross.birney
O.~Birnholtz,$^{10}$  %ofek.birnholtz
S.~Biscans,$^{1,15}$  %sebastien.biscans
S.~Biscoveanu,$^{63,6}$  %sylvia.biscoveanu
A.~Bisht,$^{22}$  %aparna.bisht
M.~Bitossi,$^{30,24}$ %massimiliano.bitossi
C.~Biwer,$^{44}$  %christopher.biwer
M.~A.~Bizouard,$^{28}$ %marieanne.bizouard
J.~K.~Blackburn,$^{1}$  %kent.blackburn
J.~Blackman,$^{48}$  %jonathan.blackman
C.~D.~Blair,$^{1,64}$  %carl.blair
D.~G.~Blair,$^{64}$  %david.blair
R.~M.~Blair,$^{47}$  %ryan.blair
S.~Bloemen,$^{65}$ %steven.bloemen
O.~Bock,$^{10}$  %oliver.bock
N.~Bode,$^{10}$  %nina.bode
M.~Boer,$^{66}$ %michel.boer
G.~Bogaert,$^{66}$ %gilles.bogaert
A.~Bohe,$^{38}$  %alejandro.bohe
F.~Bondu,$^{67}$ %francois.bondu
E.~Bonilla,$^{51}$  %edgard.bonilla
R.~Bonnand,$^{8}$ %romain.bonnand
B.~A.~Boom,$^{14}$ %boris.boom
R.~Bork,$^{1}$  %rolf.bork
V.~Boschi,$^{30,24}$ %valerio.boschi
S.~Bose,$^{68,19}$  %sukanta.bose
K.~Bossie,$^{7}$  %ken.bossie
Y.~Bouffanais,$^{39}$ %yann.bouffanais
A.~Bozzi,$^{30}$ %antonella.bozzi
C.~Bradaschia,$^{24}$ %carlo.bradaschia
P.~R.~Brady,$^{21}$  %patrick.brady
M.~Branchesi,$^{17,18}$ %marica.branchesi
J.~E.~Brau,$^{69}$   %jim.brau
T.~Briant,$^{70}$ %tristan.briant
A.~Brillet,$^{66}$ %alain.brillet
M.~Brinkmann,$^{10}$  %marc.brinkmann
V.~Brisson,$^{28}$ %violette.brisson
P.~Brockill,$^{21}$  %patrick.brockill
J.~E.~Broida,$^{71}$  %jacob.broida
A.~F.~Brooks,$^{1}$  %aidan.brooks
D.~A.~Brown,$^{44}$  %duncan.brown
D.~D.~Brown,$^{72}$  %daniel.brown
S.~Brunett,$^{1}$  %sharon.brunett
C.~C.~Buchanan,$^{2}$  %christopher.buchanan
A.~Buikema,$^{15}$  %aaron.buikema
T.~Bulik,$^{73}$ %tomasz.bulik
H.~J.~Bulten,$^{74,14}$ %henk.bulten
A.~Buonanno,$^{38,75}$  %alessandra.buonanno
D.~Buskulic,$^{8}$ %damir.buskulic
C.~Buy,$^{39}$ %christelle.buy
R.~L.~Byer,$^{51}$ %robert.byer
M.~Cabero,$^{10}$  %miriam.cabero
L.~Cadonati,$^{76}$  %laura.cadonati
G.~Cagnoli,$^{26,77}$ %giampietro.cagnoli
C.~Cahillane,$^{1}$  %craig.cahillane
J.~Calder\'on~Bustillo,$^{76}$  %juan.calderonbustillo
T.~A.~Callister,$^{1}$  %thomas.callister
E.~Calloni,$^{78,4}$ %enrico.calloni
J.~B.~Camp,$^{79}$  %jordan.camp
M.~Canepa,$^{80,59}$ %maurizio.canepa
P.~Canizares,$^{65}$ %priscilla.canizares
K.~C.~Cannon,$^{81}$  %kipp.cannon
H.~Cao,$^{72}$  %huy-tuong.cao
J.~Cao,$^{82}$  %junwei.cao
C.~D.~Capano,$^{10}$  %collin.capano
E.~Capocasa,$^{39}$ %eleonora.capocasa
F.~Carbognani,$^{30}$ %franco.carbognani
S.~Caride,$^{83}$  %santiago.caride
M.~F.~Carney,$^{84}$  %matthew.carney
J.~Casanueva~Diaz,$^{28}$ %julia.casanueva
C.~Casentini,$^{32,33}$ %claudio.casentini
S.~Caudill,$^{21,14}$  %sarah.caudill
M.~Cavagli\`a,$^{11}$  %marco.cavaglia
F.~Cavalier,$^{28}$ %fabien.cavalier
R.~Cavalieri,$^{30}$ %roberto.cavalieri
G.~Cella,$^{24}$ %giancarlo.cella
C.~B.~Cepeda,$^{1}$  %christian.cepeda
P.~Cerd\'a-Dur\'an,$^{85}$ %pablo.cerda-duran
G.~Cerretani,$^{23,24}$ %giovanni.cerretani
E.~Cesarini,$^{86,33}$ %elisabetta.cesarini
S.~J.~Chamberlin,$^{63}$  %sydney.chamberlin
M.~Chan,$^{46}$  %manleong.chan
S.~Chao,$^{87}$  %shiuh.chao
P.~Charlton,$^{88}$  %philip.charlton
E.~Chase,$^{89}$  %eve.chase
E.~Chassande-Mottin,$^{39}$ %eric.chassandemottin
D.~Chatterjee,$^{21}$  %deep.chatterjee
B.~D.~Cheeseboro,$^{41}$  %belinda.cheeseboro
H.~Y.~Chen,$^{90}$  %hsin-yu.chen
X.~Chen,$^{64}$  %xu.chen
Y.~Chen,$^{48}$  %yanbei.chen
H.-P.~Cheng,$^{5}$  %hai-ping.cheng
H.~Chia,$^{5}$  %hanyu.chia
A.~Chincarini,$^{59}$ %andrea.chincarini
A.~Chiummo,$^{30}$ %antonino.chiummo
T.~Chmiel,$^{84}$  %theresa.chmiel
H.~S.~Cho,$^{91}$  %heesuk.cho
M.~Cho,$^{75}$  %min-a.cho
J.~H.~Chow,$^{25}$  %jong.chow
N.~Christensen,$^{71,66}$ %nelson.christensen
Q.~Chu,$^{64}$  %qi.chu
A.~J.~K.~Chua,$^{13}$  %alvin.chua
S.~Chua,$^{70}$ %sheon.chua
A.~K.~W.~Chung,$^{92}$  %ka-wai.chung
S.~Chung,$^{64}$  %shinkee.chung
G.~Ciani,$^{5,53,54}$ %giacomo.ciani
R.~Ciolfi,$^{93,94}$ %riccardo.ciolfi
C.~E.~Cirelli,$^{51}$  %carissa.cirelli
A.~Cirone,$^{80,59}$ %alessio.cirone
F.~Clara,$^{47}$  %filiberto.clara
J.~A.~Clark,$^{76}$  %james.clark
P.~Clearwater,$^{95}$  %patrick.clearwater
F.~Cleva,$^{66}$ %frederic.cleva
C.~Cocchieri,$^{11}$  %camillo.cocchieri
E.~Coccia,$^{17,18}$ %eugenio.coccia
P.-F.~Cohadon,$^{70}$ %pierre-francois.cohadon
D.~Cohen,$^{28}$ %david.cohen
A.~Colla,$^{96,35}$ %alberto.colla
C.~G.~Collette,$^{97}$  %christophe.collette
L.~R.~Cominsky,$^{98}$  %lynn.cominsky
M.~Constancio~Jr.,$^{16}$  %marcio.constancio
L.~Conti,$^{54}$ %livia.conti
S.~J.~Cooper,$^{58}$  %sam.cooper
P.~Corban,$^{7}$  %paul.corban
T.~R.~Corbitt,$^{2}$  %thomas.corbitt
I.~Cordero-Carri\'on,$^{99}$ %isabel.cordero-carrion
K.~R.~Corley,$^{50}$  %kenneth.corley
N.~Cornish,$^{100}$  %neil.cornish
A.~Corsi,$^{83}$  %alessandra.corsi
S.~Cortese,$^{30}$ %stefano.cortese
C.~A.~Costa,$^{16}$  %cesar.costa
M.~W.~Coughlin,$^{71,1}$  %michael.coughlin
S.~B.~Coughlin,$^{89}$  %scott.coughlin
J.-P.~Coulon,$^{66}$ %jeanpierre.coulon
S.~T.~Countryman,$^{50}$  %stefan.countryman
P.~Couvares,$^{1}$  %peter.couvares
P.~B.~Covas,$^{101}$  %pep.covas
E.~E.~Cowan,$^{76}$  %erika.cowan
D.~M.~Coward,$^{64}$  %david.coward
M.~J.~Cowart,$^{7}$  %matthew.cowart
D.~C.~Coyne,$^{1}$  %dennis.coyne
R.~Coyne,$^{83}$  %robert.coyne
J.~D.~E.~Creighton,$^{21}$  %jolien.creighton
T.~D.~Creighton,$^{102}$  %teviet.creighton
J.~Cripe,$^{2}$  %jonathan.cripe
S.~G.~Crowder,$^{103}$  %sgwynne.crowder
T.~J.~Cullen,$^{29,2}$  %torrey.cullen
A.~Cumming,$^{46}$  %alan.cumming
L.~Cunningham,$^{46}$  %liam.cunningham
E.~Cuoco,$^{30}$ %elena.cuoco
T.~Dal~Canton,$^{79}$  %tito.canton
G.~D\'alya,$^{55}$  %gergely.dalya
S.~L.~Danilishin,$^{22,10}$  %stefan.danilishin
S.~D'Antonio,$^{33}$ %sabrina.dantonio
K.~Danzmann,$^{22,10}$  %karsten.danzmann
A.~Dasgupta,$^{104}$  %arnab.dasgupta
C.~F.~Da~Silva~Costa,$^{5}$  %filipe.dasilva
V.~Dattilo,$^{30}$ %vincenzo.dattilo
I.~Dave,$^{60}$  %ishant.dave
M.~Davier,$^{28}$ %michel.davier
D.~Davis,$^{44}$  %derek.davis
E.~J.~Daw,$^{105}$  %edward.daw
B.~Day,$^{76}$  %brian.day
S.~De,$^{44}$  %soumi.de
D.~DeBra,$^{51}$  %dan.debra
J.~Degallaix,$^{26}$ %jerome.degallaix
M.~De~Laurentis,$^{17,4}$ %martina.delaurentis
S.~Del\'eglise,$^{70}$ %samuel.deleglise
W.~Del~Pozzo,$^{58,23,24}$ %walter.delpozzo
N.~Demos,$^{15}$  %nicholas.demos
T.~Denker,$^{10}$  %timo.denker
T.~Dent,$^{10}$  %thomas.dent
R.~De~Pietri,$^{106,107}$ %roberto.depietri
V.~Dergachev,$^{38}$  %vladimir.dergachev
R.~De~Rosa,$^{78,4}$ %rosario.derosa
R.~T.~DeRosa,$^{7}$  %ryan.derosa
C.~De~Rossi,$^{26,30}$ %
R.~DeSalvo,$^{108}$  %riccardo.desalvo
O.~de~Varona,$^{10}$  %omar.de-varona
J.~Devenson,$^{27}$  %jan.devenson
S.~Dhurandhar,$^{19}$  %sanjeev.dhurandhar
M.~C.~D\'{\i}az,$^{102}$  %mario.diaz
L.~Di~Fiore,$^{4}$ %luciano.difiore
M.~Di~Giovanni,$^{109,94}$ %matteo.digiovanni
T.~Di~Girolamo,$^{50,78,4}$ %tristano.digirolamo
A.~Di~Lieto,$^{23,24}$ %alberto.dilieto
S.~Di~Pace,$^{96,35}$ %sibilla.dipace
I.~Di~Palma,$^{96,35}$ %irene.dipalma
F.~Di~Renzo,$^{23,24}$ %francesco.direnzo
Z.~Doctor,$^{90}$  %zoheyr.doctor
V.~Dolique,$^{26}$ %vincent.dolique
F.~Donovan,$^{15}$  %fred.donovan
K.~L.~Dooley,$^{11}$  %katherine.dooley
S.~Doravari,$^{10}$  %suresh.doravari
I.~Dorrington,$^{36}$  %iain.dorrington
R.~Douglas,$^{46}$  %rebecca.douglas
M.~Dovale~\'Alvarez,$^{58}$  %miguel.dovale
T.~P.~Downes,$^{21}$  %thomas.downes
M.~Drago,$^{10}$  %marco.drago
C.~Dreissigacker,$^{10}$  %christoph.dreissigacker
J.~C.~Driggers,$^{47}$  %jenne.driggers
Z.~Du,$^{82}$  %zhihui.du
M.~Ducrot,$^{8}$ %marine.ducrot
P.~Dupej,$^{46}$  %peter.dupej
S.~E.~Dwyer,$^{47}$  %sheila.dwyer
T.~B.~Edo,$^{105}$  %tega.edo
M.~C.~Edwards,$^{71}$  %matthew.edwards
A.~Effler,$^{7}$  %anamaria.effler
H.-B.~Eggenstein,$^{38,10}$  %heinz-bernd.eggenstein
P.~Ehrens,$^{1}$  %phil.ehrens
J.~Eichholz,$^{1}$  %johannes.eichholz
S.~S.~Eikenberry,$^{5}$  %stephen.eikenberry
R.~A.~Eisenstein,$^{15}$  %robert.eisenstein
R.~C.~Essick,$^{15}$  %reed.essick
D.~Estevez,$^{8}$ %dimitri.estevez
Z.~B.~Etienne,$^{41}$ %zachariah.etienne
T.~Etzel,$^{1}$  %todd.etzel
M.~Evans,$^{15}$  %matthew.evans
T.~M.~Evans,$^{7}$  %tom.evans
M.~Factourovich,$^{50}$  %maxim.factourovich
V.~Fafone,$^{32,33,17}$ %viviana.fafone
H.~Fair,$^{44}$  %hannah.fair
S.~Fairhurst,$^{36}$  %stephen.fairhurst
X.~Fan,$^{82}$  %xilong.fan
S.~Farinon,$^{59}$ %stefania.farinon
B.~Farr,$^{90}$  %benjamin.farr
W.~M.~Farr,$^{58}$  %will.farr
E.~J.~Fauchon-Jones,$^{36}$  %edward.fauchon-jones
M.~Favata,$^{110}$  %marc.favata
M.~Fays,$^{36}$  %maxime.fays
C.~Fee,$^{84}$  %campbell.fee
H.~Fehrmann,$^{10}$  %henning.fehrmann
J.~Feicht,$^{1}$  %jon.feicht
M.~M.~Fejer,$^{51}$ %martin.fejer
A.~Fernandez-Galiana,$^{15}$	%alvaro.fernandez-galiana
I.~Ferrante,$^{23,24}$ %isidoro.ferrante
E.~C.~Ferreira,$^{16}$  %elvis.ferreira
F.~Ferrini,$^{30}$ %federico.ferrini
F.~Fidecaro,$^{23,24}$ %francesco.fidecaro
D.~Finstad,$^{44}$  %daniel.finstad
I.~Fiori,$^{30}$ %irene.fiori
D.~Fiorucci,$^{39}$ %donatella.fiorucci
M.~Fishbach,$^{90}$  %maya.fishbach
R.~P.~Fisher,$^{44}$  %ryan.fisher
M.~Fitz-Axen,$^{45}$  %margot.fitz-axen
R.~Flaminio,$^{26,111}$ %raffaele.flaminio
M.~Fletcher,$^{46}$  %mark.fletcher
H.~Fong,$^{112}$  %heather.fong
J.~A.~Font,$^{85,113}$ %antonio.font
P.~W.~F.~Forsyth,$^{25}$  %perry.forsyth
S.~S.~Forsyth,$^{76}$  %steven.forsyth
J.-D.~Fournier,$^{66}$ %jean-daniel.fournier
S.~Frasca,$^{96,35}$ %sergio.frasca
F.~Frasconi,$^{24}$ %franco.frasconi
Z.~Frei,$^{55}$  %zsolt.frei
A.~Freise,$^{58}$  %andreas.freise
R.~Frey,$^{69}$  %raymond.frey
V.~Frey,$^{28}$ %valentin.frey
E.~M.~Fries,$^{1}$  %eric.fries
P.~Fritschel,$^{15}$  %peter.fritschel
V.~V.~Frolov,$^{7}$  %valery.frolov
P.~Fulda,$^{5}$  %paul.fulda
M.~Fyffe,$^{7}$  %michael.fyffe
H.~Gabbard,$^{46}$  %hunter.gabbard
B.~U.~Gadre,$^{19}$  %bhooshan.gadre
S.~M.~Gaebel,$^{58}$  %sebastian.gaebel
J.~R.~Gair,$^{114}$  %jonathan.gair
L.~Gammaitoni,$^{42}$ %luca.gammaitoni
M.~R.~Ganija,$^{72}$  %miftar.ganija
S.~G.~Gaonkar,$^{19}$  %sharad.gaonkar
C.~Garcia-Quiros,$^{101}$  %cecilio.garcia-quiros
F.~Garufi,$^{78,4}$ %fabio.garufi
B.~Gateley,$^{47}$ 
S.~Gaudio,$^{37}$  %sergio.gaudio
G.~Gaur,$^{115}$  %gurudatt.gaur
V.~Gayathri,$^{116}$  %gayathri.v
N.~Gehrels$^{\dag}$,$^{79}$  %neil.gehrels
G.~Gemme,$^{59}$ %gianluca.gemme
E.~Genin,$^{30}$ %eric.genin
A.~Gennai,$^{24}$ %alberto.gennai
D.~George,$^{12}$  %daniel.george
J.~George,$^{60}$  %jogy.george
L.~Gergely,$^{117}$  %laszlo.gergely
V.~Germain,$^{8}$ %vincent.germain
S.~Ghonge,$^{76}$  %sudarshan.ghonge
Abhirup~Ghosh,$^{20}$  %abhirup.ghosh
Archisman~Ghosh,$^{20,14}$  %archisman.ghosh
S.~Ghosh,$^{65,14,21}$ %shaon.ghosh
J.~A.~Giaime,$^{2,7}$  %joe.giaime
K.~D.~Giardina,$^{7}$  %dwayne.giardina
A.~Giazotto,$^{24}$ %adalberto.giazotto
K.~Gill,$^{37}$  %kiranjyot.gill
L.~Glover,$^{108}$  %lamar.glover
E.~Goetz,$^{118}$  %evan.goetz
R.~Goetz,$^{5}$  %ryan.goetz
S.~Gomes,$^{36}$  %sandra.gomes
B.~Goncharov,$^{6}$  %boris.goncharov
G.~Gonz\'alez,$^{2}$  %gabriela.gonzalez
J.~M.~Gonzalez~Castro,$^{23,24}$ %jose.gonzalez
A.~Gopakumar,$^{119}$  %gopakumar.achamveedu
M.~L.~Gorodetsky,$^{61}$  %michael.gorodetsky
S.~E.~Gossan,$^{1}$  %sarah.gossan
M.~Gosselin,$^{30}$ %matthieu.gosselin
R.~Gouaty,$^{8}$ %romain.gouaty
A.~Grado,$^{120,4}$ %aniello.grado
C.~Graef,$^{46}$  %christian.graef
M.~Granata,$^{26}$ %massimo.granata
A.~Grant,$^{46}$  %alastair.grant
S.~Gras,$^{15}$  %slawomir.gras
C.~Gray,$^{47}$  %corey.gray
G.~Greco,$^{121,122}$ %giuseppe.greco
A.~C.~Green,$^{58}$  %anna.green
E.~M.~Gretarsson,$^{37}$  %elizabeth.gretarsson
P.~Groot,$^{65}$ %paul.groot
H.~Grote,$^{10}$  %hartmut.grote
S.~Grunewald,$^{38}$  %steffen.grunewald
P.~Gruning,$^{28}$ %pierre.gruning
G.~M.~Guidi,$^{121,122}$ %gianluca.guidi
X.~Guo,$^{82}$  %xiangyu.guo
A.~Gupta,$^{63}$  %anuradha.gupta
M.~K.~Gupta,$^{104}$  %manojipr.gupta
K.~E.~Gushwa,$^{1}$  %kaitlin.gushwa
E.~K.~Gustafson,$^{1}$  %eric.gustafson
R.~Gustafson,$^{118}$  %dick.gustafson
O.~Halim,$^{18,17}$ %
B.~R.~Hall,$^{68}$  %bernard.hall
E.~D.~Hall,$^{15}$  %evan.hall
E.~Z.~Hamilton,$^{36}$  %eleanor.hamilton
G.~Hammond,$^{46}$  %giles.hammond
M.~Haney,$^{123}$  %maria.haney
M.~M.~Hanke,$^{10}$  %manuela.hanke
J.~Hanks,$^{47}$  %jonathan.hanks
C.~Hanna,$^{63}$  %chad.hanna
M.~D.~Hannam,$^{36}$  %mark.hannam
O.~A.~Hannuksela,$^{92}$  %otto.hannuksela
J.~Hanson,$^{7}$  %joe.hanson
T.~Hardwick,$^{2}$  %terra.hardwick
J.~Harms,$^{17,18}$ %jan.harms
G.~M.~Harry,$^{124}$  %gregg.harry
I.~W.~Harry,$^{38}$  %ian.harry
M.~J.~Hart,$^{46}$  %martin.hart
C.-J.~Haster,$^{112}$  %carl-johan.haster
K.~Haughian,$^{46}$  %karen.haughian
J.~Healy,$^{57}$  %james.healy
A.~Heidmann,$^{70}$ %antoine.heidmann
M.~C.~Heintze,$^{7}$  %matthew.heintze
H.~Heitmann,$^{66}$ %henrich.heitmann
P.~Hello,$^{28}$ %patrice.hello
G.~Hemming,$^{30}$ %gary.hemming
M.~Hendry,$^{46}$  %martin.hendry
I.~S.~Heng,$^{46}$  %siong.heng
J.~Hennig,$^{46}$  %jan-simon.hennig
A.~W.~Heptonstall,$^{1}$  %alastair.heptonstall
M.~Heurs,$^{10,22}$  %michele.heurs
S.~Hild,$^{46}$  %stefan.hild
T.~Hinderer,$^{65}$ %tanja.hinderer
D.~Hoak,$^{30}$ %daniel.hoak
D.~Hofman,$^{26}$ %david.hofman
K.~Holt,$^{7}$  %kathy.holt
D.~E.~Holz,$^{90}$  %daniel.holz
P.~Hopkins,$^{36}$  %paul.hopkins
C.~Horst,$^{21}$  %christian.horst
J.~Hough,$^{46}$  %james.hough
E.~A.~Houston,$^{46}$  %ewan.houston
E.~J.~Howell,$^{64}$  %eric.howell
A.~Hreibi,$^{66}$ 
Y.~M.~Hu,$^{10}$  %yiming.hu
E.~A.~Huerta,$^{12}$  %eliu.huerta
D.~Huet,$^{28}$ %dominique.huet
B.~Hughey,$^{37}$  %brennan.hughey
S.~Husa,$^{101}$  %sascha.husa
S.~H.~Huttner,$^{46}$  %sabina.huttner
T.~Huynh-Dinh,$^{7}$  %tien.huynh-dinh
N.~Indik,$^{10}$  %nathaniel.indik
R.~Inta,$^{83}$  %ra.inta
G.~Intini,$^{96,35}$ %giuseppe.intini
H.~N.~Isa,$^{46}$  %hafizah.isa
J.-M.~Isac,$^{70}$ %
M.~Isi,$^{1}$  %max.isi
B.~R.~Iyer,$^{20}$  %bala.iyer
K.~Izumi,$^{47}$  %kiwamu.izumi
T.~Jacqmin,$^{70}$ %thibaut.jacqmin
K.~Jani,$^{76}$  %karan.jani
P.~Jaranowski,$^{125}$ %piotr.jaranowski
S.~Jawahar,$^{62}$  %sharat.jawahar
F.~Jim\'enez-Forteza,$^{101}$  %francisco.forteza
W.~W.~Johnson,$^{2}$  %warren.johnson
D.~I.~Jones,$^{126}$  %ian.jones
R.~Jones,$^{46}$  %russell.jones
R.~J.~G.~Jonker,$^{14}$ %reinier.jonker
L.~Ju,$^{64}$  %ju.li
J.~Junker,$^{10}$  %jonas.junker
C.~V.~Kalaghatgi,$^{36}$  %chinmay.kalaghatgi
V.~Kalogera,$^{89}$  %vassiliki.kalogera
B.~Kamai,$^{1}$
S.~Kandhasamy,$^{7}$  %shivaraj.kandhasamy
G.~Kang,$^{40}$  %gungwon.kang
J.~B.~Kanner,$^{1}$  %jonah.kanner
S.~J.~Kapadia,$^{21}$  %shasvath.kapadia
S.~Karki,$^{69}$  %sudarshan.karki
K.~S.~Karvinen,$^{10}$	%kai.karvinen
M.~Kasprzack,$^{2}$  %marie.kasprzack
M.~Katolik,$^{12}$  %michael.katolik
E.~Katsavounidis,$^{15}$  %erik.katsavounidis
W.~Katzman,$^{7}$  %william.katzman
S.~Kaufer,$^{22}$  %steffen.kaufer
K.~Kawabe,$^{47}$  %keita.kawabe
F.~K\'ef\'elian,$^{66}$ %fabien.kefelian
D.~Keitel,$^{46}$  %david.keitel
A.~J.~Kemball,$^{12}$  %athol.kemball
R.~Kennedy,$^{105}$  %ross.kennedy
C.~Kent,$^{36}$  %christopher.kent
J.~S.~Key,$^{127}$  %joey.key
F.~Y.~Khalili,$^{61}$  %farit.khalili
I.~Khan,$^{17,33}$ %
S.~Khan,$^{10}$  %sebastian.khan
Z.~Khan,$^{104}$  %ziauddin.khan
E.~A.~Khazanov,$^{128}$  %efim.khazanov
N.~Kijbunchoo,$^{25}$  %nutsinee.kijbunchoo
Chunglee~Kim,$^{129}$  %chunglee.kim
J.~C.~Kim,$^{130}$  %jeongcho.kim
K.~Kim,$^{92}$  %kyungmin.kim
W.~Kim,$^{72}$  %won.kim
W.~S.~Kim,$^{131}$  %whansun.kim
Y.-M.~Kim,$^{91}$  %young-min.kim
S.~J.~Kimbrell,$^{76}$  %seth.kimbrell
E.~J.~King,$^{72}$  %eleanor.king
P.~J.~King,$^{47}$  %peter.king
M.~Kinley-Hanlon,$^{124}$  %maya.kinley-hanon
R.~Kirchhoff,$^{10}$  %robin.kirchhoff
J.~S.~Kissel,$^{47}$  %jeffrey.kissel
L.~Kleybolte,$^{34}$  %lisa.kleybolte
S.~Klimenko,$^{5}$  %sergei.klimenko
T.~D.~Knowles,$^{41}$	%tyler.knowles
P.~Koch,$^{10}$  %philip.koch
S.~M.~Koehlenbeck,$^{10}$  %sina.koehlenbeck
S.~Koley,$^{14}$ %soumen.koley
V.~Kondrashov,$^{1}$  %veronica.kondrashov
A.~Kontos,$^{15}$  %antonios.kontos
M.~Korobko,$^{34}$  %mikhail.korobko
W.~Z.~Korth,$^{1}$  %william.korth
I.~Kowalska,$^{73}$ %izabela.kowalska
D.~B.~Kozak,$^{1}$  %dan.kozak
C.~Kr\"amer,$^{10}$  %christina.krmer
V.~Kringel,$^{10}$  %volker.kringel
B.~Krishnan,$^{10}$  %badri.krishnan
A.~Kr\'olak,$^{132,133}$ %andrzej.krolak
G.~Kuehn,$^{10}$  %gerrit.kuehn
P.~Kumar,$^{112}$  %prayush.kumar
R.~Kumar,$^{104}$  %rakesh.kumar
S.~Kumar,$^{20}$  %sumit.kumar
L.~Kuo,$^{87}$  %ling-chi.kuo
A.~Kutynia,$^{132}$ %adam.kutynia
S.~Kwang,$^{21}$  %shawn.kwang
B.~D.~Lackey,$^{38}$  %benjamin.lackey
K.~H.~Lai,$^{92}$  %kwun-hang.lai
M.~Landry,$^{47}$  %michael.landry
R.~N.~Lang,$^{134}$  %ryan.lang
J.~Lange,$^{57}$  %jacob.lange
B.~Lantz,$^{51}$  %brian.lantz
R.~K.~Lanza,$^{15}$  %robert.lanza
A.~Lartaux-Vollard,$^{28}$ %angelique.vollard
P.~D.~Lasky,$^{6}$  %paul.lasky
M.~Laxen,$^{7}$  %michael.laxen
A.~Lazzarini,$^{1}$  %albert.lazzarini
C.~Lazzaro,$^{54}$ %claudia.lazzaro
P.~Leaci,$^{96,35}$ %paola.leaci
S.~Leavey,$^{46}$  %sean.leavey
C.~H.~Lee,$^{91}$  %chang-hwan.lee
H.~K.~Lee,$^{135}$  %hyunkyu.lee
H.~M.~Lee,$^{136}$  %hyung-mok.lee
H.~W.~Lee,$^{130}$  %hyungwon.lee
K.~Lee,$^{46}$  %kyung-ha.lee
J.~Lehmann,$^{10}$  %johannes.lehmann
A.~Lenon,$^{41}$  %amber.lenon
M.~Leonardi,$^{109,94}$ %matteo.leonardi
N.~Leroy,$^{28}$ %nicolas.leroy
N.~Letendre,$^{8}$ %nicolas.letendre
Y.~Levin,$^{6}$  %yuri.levin
T.~G.~F.~Li,$^{92}$  %tjonnie.li
S.~D.~Linker,$^{108}$  %seth.linker
T.~B.~Littenberg,$^{137}$  %tyson.littenberg
J.~Liu,$^{64}$  %liu.jian
R.~K.~L.~Lo,$^{92}$  %ka-lok.lo
N.~A.~Lockerbie,$^{62}$  %nick.lockerbie
L.~T.~London,$^{36}$  %lionel.london
J.~E.~Lord,$^{44}$  %jaysin.lord
M.~Lorenzini,$^{17,18}$ %matteo.lorenzini
V.~Loriette,$^{138}$ %vincent.loriette
M.~Lormand,$^{7}$  %marc.lormand
G.~Losurdo,$^{24}$ %giovanni.losurdo
J.~D.~Lough,$^{10}$  %james.lough
C.~O.~Lousto,$^{57}$  %carlos.lousto
G.~Lovelace,$^{29}$  %geoffrey.lovelace
H.~L\"uck,$^{22,10}$  %harald.lueck
D.~Lumaca,$^{32,33}$ %diana.lumaca
A.~P.~Lundgren,$^{10}$  %andrew.lundgren
R.~Lynch,$^{15}$  %ryan.lynch
Y.~Ma,$^{48}$  %ma.yiqiu
R.~Macas,$^{36}$  %ronaldas.macas
S.~Macfoy,$^{27}$  %sean.macfoy
B.~Machenschalk,$^{10}$  %bernd.machenschalk
M.~MacInnis,$^{15}$  %myron.macinnis
D.~M.~Macleod,$^{36}$  %duncan.macleod
I.~Maga\~na~Hernandez,$^{21}$  %ignacio.magana
F.~Maga\~na-Sandoval,$^{44}$  %fabian.magana-sandoval
L.~Maga\~na~Zertuche,$^{44}$  %lorena.magana-zertuche
R.~M.~Magee,$^{63}$  %ryan.magee
E.~Majorana,$^{35}$ %ettore.majorana
I.~Maksimovic,$^{138}$ %ivan.maksimovic
N.~Man,$^{66}$ %catherine.man
V.~Mandic,$^{45}$  %vuk.mandic
V.~Mangano,$^{46}$  %valentina.mangano
G.~L.~Mansell,$^{25}$  %georgia.mansell
M.~Manske,$^{21,25}$  %michael.manske
M.~Mantovani,$^{30}$ %maddalena.mantovani
F.~Marchesoni,$^{52,43}$ %fabio.marchesoni
F.~Marion,$^{8}$ %frederique.marion
S.~M\'arka,$^{50}$  %szabolcs.marka
Z.~M\'arka,$^{50}$  %zsuzsanna.marka
C.~Markakis,$^{12}$  %charalampos.markakis
A.~S.~Markosyan,$^{51}$  %ashot.markosyan
A.~Markowitz,$^{1}$  %aaron.markowitz
E.~Maros,$^{1}$  %ed.maros
A.~Marquina,$^{99}$ %antonio.marquina
F.~Martelli,$^{121,122}$ %filippo.martelli
L.~Martellini,$^{66}$ %lionel.martellini
I.~W.~Martin,$^{46}$  %ian.martin
R.~M.~Martin,$^{110}$  	%rodica.martin
D.~V.~Martynov,$^{15}$  %denis.martynov
K.~Mason,$^{15}$  %ken.mason
E.~Massera,$^{105}$  %elena.massera
A.~Masserot,$^{8}$ %alain.masserot
T.~J.~Massinger,$^{1}$  %thomas.massinger
M.~Masso-Reid,$^{46}$  %mariela.masso-reid
S.~Mastrogiovanni,$^{96,35}$ %simone.mastrogiovanni
A.~Matas,$^{45}$  %andrew.matas
F.~Matichard,$^{1,15}$  %fabrice.matichard
L.~Matone,$^{50}$  %luca.matone
N.~Mavalvala,$^{15}$  %nergis.mavalvala
N.~Mazumder,$^{68}$  %nairwita.mazumder
R.~McCarthy,$^{47}$  %richard.mccarthy
D.~E.~McClelland,$^{25}$  %david.mcclelland
S.~McCormick,$^{7}$  %scott.mccormick
L.~McCuller,$^{15}$  %lee.mcculler
S.~C.~McGuire,$^{139}$  %stephen.mcguire
G.~McIntyre,$^{1}$  %gary.mcintyre
J.~McIver,$^{1}$  %jessica.mciver
D.~J.~McManus,$^{25}$  %david.mcmanus
L.~McNeill,$^{6}$  %lucy.mcneill
T.~McRae,$^{25}$  %terry.mcrae
S.~T.~McWilliams,$^{41}$  %sean.mcwilliams
D.~Meacher,$^{63}$  %duncan.meacher
G.~D.~Meadors,$^{38,10}$  %grant.meadors
M.~Mehmet,$^{10}$  %moritz.mehmet
J.~Meidam,$^{14}$ %jeroen.meidam
E.~Mejuto-Villa,$^{9}$  %elena.mejuto-villa
A.~Melatos,$^{95}$  %andrew.melatos
G.~Mendell,$^{47}$  %gregory.mendell
R.~A.~Mercer,$^{21}$  %adam.mercer
E.~L.~Merilh,$^{47}$  %edmond.merilh
M.~Merzougui,$^{66}$ %mourad.merzougui
S.~Meshkov,$^{1}$  %syd.meshkov
C.~Messenger,$^{46}$  %chris.messenger
C.~Messick,$^{63}$  %cody.messick
R.~Metzdorff,$^{70}$ %
P.~M.~Meyers,$^{45}$  %patrick.meyers
H.~Miao,$^{58}$  %haixing.miao
C.~Michel,$^{26}$ %christophe.michel
H.~Middleton,$^{58}$  %hannah.middleton
E.~E.~Mikhailov,$^{140}$  %eugeniy.mikhailov
L.~Milano,$^{78,4}$ %leopoldo.milano
A.~L.~Miller,$^{5,96,35}$  %andrewlawrence.miller
B.~B.~Miller,$^{89}$  %brandon.miller
J.~Miller,$^{15}$	%john.miller
M.~Millhouse,$^{100}$  %meg.millhouse
M.~C.~Milovich-Goff,$^{108}$  %michael.milovich-goff
O.~Minazzoli,$^{66,141}$ %olivier.minazzoli
Y.~Minenkov,$^{33}$ %yuri.minenkov
J.~Ming,$^{38}$  %jing.ming
C.~Mishra,$^{142}$  %chandra.mishra
S.~Mitra,$^{19}$  %sanjit.mitra
V.~P.~Mitrofanov,$^{61}$  %valery.mitrofanov
G.~Mitselmakher,$^{5}$ %guenakh.mitselmakher
R.~Mittleman,$^{15}$  %richard.mittleman
D.~Moffa,$^{84}$  %donald.moffa
A.~Moggi,$^{24}$ %andrea.moggi
K.~Mogushi,$^{11}$  %kentaro.mogushi
M.~Mohan,$^{30}$ %martin.mohan
S.~R.~P.~Mohapatra,$^{15}$  %satyanarayan.raypitambarmohapatra
M.~Montani,$^{121,122}$ %matteo.montani
C.~J.~Moore,$^{13}$  %christopher.moore
D.~Moraru,$^{47}$  %dan.moraru
G.~Moreno,$^{47}$  %gerardo.moreno
S.~R.~Morriss,$^{102}$  %sean.morriss
B.~Mours,$^{8}$ %benoit.mours
C.~M.~Mow-Lowry,$^{58}$  %conor.mow-lowry
G.~Mueller,$^{5}$  %guido.mueller
A.~W.~Muir,$^{36}$  %alistair.muir
Arunava~Mukherjee,$^{10}$  %arunava.mukherjee
D.~Mukherjee,$^{21}$  %debnandini.mukherjee
S.~Mukherjee,$^{102}$  %soma.mukherjee
N.~Mukund,$^{19}$  %nikhil.mukund
A.~Mullavey,$^{7}$  %adam.mullavey
J.~Munch,$^{72}$  %jesper.munch
E.~A.~Mu\~niz,$^{44}$  %erik.muniz
M.~Muratore,$^{37}$  %martina.muratore
P.~G.~Murray,$^{46}$  %peter.murray
K.~Napier,$^{76}$  %kate.napier
I.~Nardecchia,$^{32,33}$ %ilaria.nardecchia
L.~Naticchioni,$^{96,35}$ %luca.naticchioni
R.~K.~Nayak,$^{143}$  %rajesh.nayak
J.~Neilson,$^{108}$  %joshua.neilson
G.~Nelemans,$^{65,14}$ %gijs.nelemans
T.~J.~N.~Nelson,$^{7}$  %timothy.nelson
M.~Nery,$^{10}$  %marina.nery
A.~Neunzert,$^{118}$  %ansel.neunzert
L.~Nevin,$^{1}$  %lydia.nevin
J.~M.~Newport,$^{124}$  %jonathan.newport
G.~Newton$^{\ddag}$,$^{46}$  %gavin.newton
K.~K.~Y.~Ng,$^{92}$  %kwan-yeung.ng
T.~T.~Nguyen,$^{25}$  %thanh.nguyen
D.~Nichols,$^{65}$ %david.nichols
A.~B.~Nielsen,$^{10}$  %alex.nielsen
S.~Nissanke,$^{65,14}$ %samaya.nissanke
A.~Nitz,$^{10}$  %alex.nitz
A.~Noack,$^{10}$  %andreas.noack
F.~Nocera,$^{30}$ %flavio.nocera
D.~Nolting,$^{7}$  %david.nolting
C.~North,$^{36}$  %chris.north
L.~K.~Nuttall,$^{36}$  %laura.nuttall
J.~Oberling,$^{47}$  %jason.oberling
G.~D.~O'Dea,$^{108}$  %greta.odea
G.~H.~Ogin,$^{144}$  %greg.ogin
J.~J.~Oh,$^{131}$  %john.oh
S.~H.~Oh,$^{131}$  %sanghoon.oh
F.~Ohme,$^{10}$  %frank.ohme
M.~A.~Okada,$^{16}$  %marcos.okada
M.~Oliver,$^{101}$  %miquel.oliver
P.~Oppermann,$^{10}$  %patrick.oppermann
Richard~J.~Oram,$^{7}$  %richard.oram
B.~O'Reilly,$^{7}$  %brian.oreilly
R.~Ormiston,$^{45}$  %rich.ormiston
L.~F.~Ortega,$^{5}$  %luis.ortega
R.~O'Shaughnessy,$^{57}$  %richard.oshaughnessy
S.~Ossokine,$^{38}$  %serguei.ossokine
D.~J.~Ottaway,$^{72}$  %david.ottaway
H.~Overmier,$^{7}$  %harry.overmier
B.~J.~Owen,$^{83}$  %ben.owen
A.~E.~Pace,$^{63}$  %alexander.pace
J.~Page,$^{137}$  %jessica.page
M.~A.~Page,$^{64}$  %michael.page
A.~Pai,$^{116,145}$  %archana.pai
S.~A.~Pai,$^{60}$  %siddhesh.pai
J.~R.~Palamos,$^{69}$  %jordan.palamos
O.~Palashov,$^{128}$  %oleg.palashov
C.~Palomba,$^{35}$ %cristiano.palomba
A.~Pal-Singh,$^{34}$  %amrit.pal-singh
Howard~Pan,$^{87}$  %howard.pan
Huang-Wei~Pan,$^{87}$  %huang-wei.pan
B.~Pang,$^{48}$  %belinda.pang
P.~T.~H.~Pang,$^{92}$  %tsun-ho.pang
C.~Pankow,$^{89}$  %chris.pankow
F.~Pannarale,$^{36}$  %francesco.pannarale
B.~C.~Pant,$^{60}$  %brijesh.pant
F.~Paoletti,$^{24}$ %federico.paoletti
A.~Paoli,$^{30}$ %andrea.paoli
M.~A.~Papa,$^{38,21,10}$  %maria.papa
A.~Parida,$^{19}$  %abhishek.parida
W.~Parker,$^{7}$  %william.parker
D.~Pascucci,$^{46}$  %daniela.pascucci
A.~Pasqualetti,$^{30}$ %antonio.pasqualetti
R.~Passaquieti,$^{23,24}$ %roberto.passaquieti
D.~Passuello,$^{24}$ %diego.passuello
M.~Patil,$^{133}$ %
B.~Patricelli,$^{146,24}$ %barbara.patricelli
B.~L.~Pearlstone,$^{46}$  %brynley.pearlstone
M.~Pedraza,$^{1}$  %mike.pedraza
R.~Pedurand,$^{26,147}$ %richard.pedurand
L.~Pekowsky,$^{44}$  %niels.versavel
A.~Pele,$^{7}$  %arnaud.pele
S.~Penn,$^{148}$  %steven.penn
C.~J.~Perez,$^{47}$  %carlos.perez
A.~Perreca,$^{1,109,94}$ %antonio.perreca
L.~M.~Perri,$^{89}$  %leah.perri
H.~P.~Pfeiffer,$^{112,38}$  %harald.pfeiffer
M.~Phelps,$^{46}$  %margot.phelps
O.~J.~Piccinni,$^{96,35}$ %ornella.piccinni
M.~Pichot,$^{66}$ %mikhael.pichot
F.~Piergiovanni,$^{121,122}$ %francesco.piergiovanni
V.~Pierro,$^{9}$  %vincenzo.pierro
G.~Pillant,$^{30}$ %gabriel.pillant
L.~Pinard,$^{26}$ %laurent.pinard
I.~M.~Pinto,$^{9}$  %innocenzo.pinto
M.~Pirello,$^{47}$  %marc.pirello
M.~Pitkin,$^{46}$  %matthew.pitkin
M.~Poe,$^{21}$  %mark.poe
R.~Poggiani,$^{23,24}$ %rosa.poggiani
P.~Popolizio,$^{30}$ %pasquale.popolizio
E.~K.~Porter,$^{39}$ %ed.porter
A.~Post,$^{10}$  %alexander.post
J.~Powell,$^{46,149}$  %jade.powell
J.~Prasad,$^{19}$  %jayanti.prasad
J.~W.~W.~Pratt,$^{37}$  %james.pratt
G.~Pratten,$^{101}$  %geraint.pratten
V.~Predoi,$^{36}$  %valeriu.predoi
T.~Prestegard,$^{21}$  %tanner.prestegard
M.~Prijatelj,$^{10}$  %mirko.prijatelj
M.~Principe,$^{9}$  %maria.principe
S.~Privitera,$^{38}$  %stephen.privitera
G.~A.~Prodi,$^{109,94}$ %giovanni.prodi
L.~G.~Prokhorov,$^{61}$  %leonid.prokhorov
O.~Puncken,$^{10}$  %oliver.puncken
M.~Punturo,$^{43}$ %michele.punturo
P.~Puppo,$^{35}$ %paola.puppo
M.~P\"urrer,$^{38}$  %michael.puerrer
H.~Qi,$^{21}$  %hong.qi
V.~Quetschke,$^{102}$  %volker.quetschke
E.~A.~Quintero,$^{1}$  %eric.quintero
R.~Quitzow-James,$^{69}$  %ryan.quitzow-james
F.~J.~Raab,$^{47}$  %fred.raab
D.~S.~Rabeling,$^{25}$  %david.rabeling
H.~Radkins,$^{47}$  %hugh.radkins
P.~Raffai,$^{55}$  %peter.raffai
S.~Raja,$^{60}$  %sendhil.raja
C.~Rajan,$^{60}$  %rajan.c
B.~Rajbhandari,$^{83}$  %binod.rajbhandari
M.~Rakhmanov,$^{102}$  %malik.rakhmanov
K.~E.~Ramirez,$^{102}$  %karla.ramirez
A.~Ramos-Buades,$^{101}$  %antoni.ramos-buades
P.~Rapagnani,$^{96,35}$ %piero.rapagnani
V.~Raymond,$^{38}$  %vivien.raymond
M.~Razzano,$^{23,24}$ %massimiliano.razzano
J.~Read,$^{29}$  %jocelyn.read
T.~Regimbau,$^{66}$ %tania.regimbau
L.~Rei,$^{59}$ %luca.rei
S.~Reid,$^{62}$  %stuart.reid
D.~H.~Reitze,$^{1,5}$  %david.reitze
W.~Ren,$^{12}$  %wei.ren
S.~D.~Reyes,$^{44}$  %steven.reyes
F.~Ricci,$^{96,35}$ %fulvio.ricci
P.~M.~Ricker,$^{12}$  %paul.ricker
S.~Rieger,$^{10}$  %sascha.rieger
K.~Riles,$^{118}$  %keith.riles
M.~Rizzo,$^{57}$  %monica.rizzo
N.~A.~Robertson,$^{1,46}$  %norna.robertson
R.~Robie,$^{46}$  %raymond.robie
F.~Robinet,$^{28}$ %florent.robinet
A.~Rocchi,$^{33}$ %alessio.rocchi
L.~Rolland,$^{8}$ %loic.rolland
J.~G.~Rollins,$^{1}$  %jameson.rollins
V.~J.~Roma,$^{69}$  %vincent.roma
J.~D.~Romano,$^{102}$  %joseph.romano %%opt-in
R.~Romano,$^{3,4}$ %rocco.romano
C.~L.~Romel,$^{47}$  %chandra.romel
J.~H.~Romie,$^{7}$  %janeen.romie
D.~Rosi\'nska,$^{150,56}$ %dorota.rosinska
M.~P.~Ross,$^{151}$  %michael.ross
S.~Rowan,$^{46}$  %sheila.rowan
A.~R\"udiger,$^{10}$  %albrecht.ruediger
P.~Ruggi,$^{30}$ %paolo.ruggi
G.~Rutins,$^{27}$  %guntis.rutins
K.~Ryan,$^{47}$  %kyle.ryan
S.~Sachdev,$^{1}$  %surabhi.sachdev
T.~Sadecki,$^{47}$  %travis.sadecki
L.~Sadeghian,$^{21}$  %laleh.sadeghian
M.~Sakellariadou,$^{152}$  %mairi.sakellariadou
L.~Salconi,$^{30}$ %livio.salconi
M.~Saleem,$^{116}$  %muhammed.saleem
F.~Salemi,$^{10}$  %francesco.salemi
A.~Samajdar,$^{143}$  %anuradha.samajdar
L.~Sammut,$^{6}$  %letizia.sammut
L.~M.~Sampson,$^{89}$  %laura.sampson
E.~J.~Sanchez,$^{1}$  %eduardo.sanchez
L.~E.~Sanchez,$^{1}$  %luis.sanchez
N.~Sanchis-Gual,$^{85}$ %nicolas.sanchis-gual
V.~Sandberg,$^{47}$  %vernon.sandberg
J.~R.~Sanders,$^{44}$  %jaclyn.sanders
B.~Sassolas,$^{26}$ %benoit.sassolas
B.~S.~Sathyaprakash,$^{63,36}$  %b.sathyaprakash
P.~R.~Saulson,$^{44}$  %peter.saulson
O.~Sauter,$^{118}$  %orion.sauter
R.~L.~Savage,$^{47}$  %richard.savage
A.~Sawadsky,$^{34}$  %andreas.sawadsky
P.~Schale,$^{69}$  %paul.schale
M.~Scheel,$^{48}$  %mark.scheel
J.~Scheuer,$^{89}$  %jacob.scheuer
J.~Schmidt,$^{10}$  %justus.schmidt
P.~Schmidt,$^{1,65}$ %patricia.schmidt
R.~Schnabel,$^{34}$  %roman.schnabel
R.~M.~S.~Schofield,$^{69}$  %robert.schofield
A.~Sch\"onbeck,$^{34}$  %axel.schoenbeck
E.~Schreiber,$^{10}$  %emil.schreiber
D.~Schuette,$^{10,22}$  %dirk.schuette
B.~W.~Schulte,$^{10}$  %bernd.schulte
B.~F.~Schutz,$^{36,10}$  %bernard.schutz
S.~G.~Schwalbe,$^{37}$  %sophia.schwalbe
J.~Scott,$^{46}$  %jamie.scott
S.~M.~Scott,$^{25}$  %susan.scott
E.~Seidel,$^{12}$  %ed.seidel
D.~Sellers,$^{7}$  %danny.sellers
A.~S.~Sengupta,$^{153}$  %anand.sengupta
D.~Sentenac,$^{30}$ %daniel.sentenac
V.~Sequino,$^{32,33,17}$ %valeria.sequino
A.~Sergeev,$^{128}$ 	%alexander.sergeev
D.~A.~Shaddock,$^{25}$  %daniel.shaddock
T.~J.~Shaffer,$^{47}$  %thomas.shaffer
A.~A.~Shah,$^{137}$  %ankur.shah
M.~S.~Shahriar,$^{89}$  %selim.shahriar
M.~B.~Shaner,$^{108}$  %morgan.shaner
L.~Shao,$^{38}$  %lijing.shao
B.~Shapiro,$^{51}$  %brett.shapiro
P.~Shawhan,$^{75}$  %peter.shawhan
A.~Sheperd,$^{21}$  %alec.sheperd
D.~H.~Shoemaker,$^{15}$  %david.shoemaker
D.~M.~Shoemaker,$^{76}$  %deirdre.shoemaker
K.~Siellez,$^{76}$  %karelle.siellez
X.~Siemens,$^{21}$  %xavier.siemens
M.~Sieniawska,$^{56}$ %magdalena.sieniawska
D.~Sigg,$^{47}$  %daniel.sigg
A.~D.~Silva,$^{16}$  %allan.silva
L.~P.~Singer,$^{79}$  %leo.singer
A.~Singh,$^{38,10,22}$  %avneet.singh
A.~Singhal,$^{17,35}$ %akshat.singhal
A.~M.~Sintes,$^{101}$  %alicia.sintes
B.~J.~J.~Slagmolen,$^{25}$  %bram.slagmolen
B.~Smith,$^{7}$  %bryan.smith
J.~R.~Smith,$^{29}$  %joshua.smith
R.~J.~E.~Smith,$^{1,6}$  %rory.smith
S.~Somala,$^{154}$  %surendranadh.somala
E.~J.~Son,$^{131}$  %edwin.son
J.~A.~Sonnenberg,$^{21}$  %jacob.sonnenberg
B.~Sorazu,$^{46}$  %borja.sorazu
F.~Sorrentino,$^{59}$ %fiodor.sorrentino
T.~Souradeep,$^{19}$  %tarun.souradeep
A.~P.~Spencer,$^{46}$  %andrew.spencer
A.~K.~Srivastava,$^{104}$  %amit.srivastava
K.~Staats,$^{37}$  %kai.staats
A.~Staley,$^{50}$  %alexan.staley
M.~Steinke,$^{10}$  %michael.steinke
J.~Steinlechner,$^{34,46}$  %jessica.steinlechner
S.~Steinlechner,$^{34}$  %sebastian.steinlechner
D.~Steinmeyer,$^{10}$  %daniel.steinmeyer
S.~P.~Stevenson,$^{58,149}$  %simon.stevenson
R.~Stone,$^{102}$  %robert.stone
D.~J.~Stops,$^{58}$  %david.stops
K.~A.~Strain,$^{46}$  %ken.strain
G.~Stratta,$^{121,122}$ %giulia.stratta
S.~E.~Strigin,$^{61}$  %sergey.strigin
A.~Strunk,$^{47}$  %amber.henry
R.~Sturani,$^{155}$  %riccardo.sturani
A.~L.~Stuver,$^{7}$  %amber.stuver
T.~Z.~Summerscales,$^{156}$  %tiffany.summerscales
L.~Sun,$^{95}$  %ling.sun
S.~Sunil,$^{104}$  %sunil.s
J.~Suresh,$^{19}$  %jishnu.suresh
P.~J.~Sutton,$^{36}$  %patrick.sutton
B.~L.~Swinkels,$^{30}$ %bas.swinkels
M.~J.~Szczepa\'nczyk,$^{37}$  %marek.szczepanczyk
M.~Tacca,$^{14}$ %matteo.tacca
S.~C.~Tait,$^{46}$  %simon.tait
C.~Talbot,$^{6}$  %colm.talbot
D.~Talukder,$^{69}$  %dipongkar.talukder
D.~B.~Tanner,$^{5}$  %david.tanner
M.~T\'apai,$^{117}$  %marton.tapai
A.~Taracchini,$^{38}$  %andrea.taracchini
J.~D.~Tasson,$^{71}$  %jay.tasson
J.~A.~Taylor,$^{137}$  %jordan.taylor
R.~Taylor,$^{1}$  %robert.taylor2
S.~V.~Tewari,$^{148}$  %shivam.tewari
T.~Theeg,$^{10}$  %thomas.theeg
F.~Thies,$^{10}$  %fabian.thies
E.~G.~Thomas,$^{58}$  %gareth.thomas
M.~Thomas,$^{7}$  %michael.thomas
P.~Thomas,$^{47}$  %patrick.thomas
K.~A.~Thorne,$^{7}$  %keith.thorne
E.~Thrane,$^{6}$  %eric.thrane
S.~Tiwari,$^{17,94}$ %shubhanshu.tiwari
V.~Tiwari,$^{36}$  %vaibhav.tiwari
K.~V.~Tokmakov,$^{62}$  %kirill.tokmakov
K.~Toland,$^{46}$  %karl.toland
M.~Tonelli,$^{23,24}$ %mauro.tonelli
Z.~Tornasi,$^{46}$  %zeno.tornasi
A.~Torres-Forn\'e,$^{85}$ %alejandro.torres
C.~I.~Torrie,$^{1}$  %calum.torrie
D.~T\"oyr\"a,$^{58}$  %daniel.toyra
F.~Travasso,$^{30,43}$ %flavio.travasso
G.~Traylor,$^{7}$  %gary.traylor
J.~Trinastic,$^{5}$  %jonathan.trinastic
M.~C.~Tringali,$^{109,94}$ %maria.tringali
L.~Trozzo,$^{157,24}$ %lucia.trozzo
K.~W.~Tsang,$^{14}$ %ka-wa.tsang
M.~Tse,$^{15}$  %maggie.tse
R.~Tso,$^{1}$  %rhondale.tso
L.~Tsukada,$^{81}$	%leo.tsukada
D.~Tsuna,$^{81}$  %daichi.tsuna
D.~Tuyenbayev,$^{102}$  %darkhan.tuyenbayev
K.~Ueno,$^{21}$  %koh.ueno
D.~Ugolini,$^{158}$  %dennis.ugolini
C.~S.~Unnikrishnan,$^{119}$  %cs.unnikrishnan
A.~L.~Urban,$^{1}$  %alexander.urban
S.~A.~Usman,$^{36}$  %samantha.usman
H.~Vahlbruch,$^{22}$  %henning.vahlbruch
G.~Vajente,$^{1}$  %gabriele.vajente
G.~Valdes,$^{2}$	%guillermo.valdes
N.~van~Bakel,$^{14}$ %niels.vanbakel
M.~van~Beuzekom,$^{14}$ %martin.beuzekom
J.~F.~J.~van~den~Brand,$^{74,14}$ %jo.vandenbrand
C.~Van~Den~Broeck,$^{14,159}$ %chris.vandenbroeck
D.~C.~Vander-Hyde,$^{44}$  %daniel.vander-hyde
L.~van~der~Schaaf,$^{14}$ %laura.van-der-schaaf
J.~V.~van~Heijningen,$^{14}$ %joris.vanheijningen
A.~A.~van~Veggel,$^{46}$  %marielle.vanveggel
M.~Vardaro,$^{53,54}$ %marco.vardaro
V.~Varma,$^{48}$  %vijay.varma
S.~Vass,$^{1}$  %steve.vass
M.~Vas\'uth,$^{49}$ %matyas.vasuth
A.~Vecchio,$^{58}$  %alberto.vecchio
G.~Vedovato,$^{54}$ %gabriele.vedovato
J.~Veitch,$^{46}$  %john.veitch
P.~J.~Veitch,$^{72}$  %peter.veitch
K.~Venkateswara,$^{151}$  %krishna.venkateswara
G.~Venugopalan,$^{1}$  %gautam.venugopalan
D.~Verkindt,$^{8}$ %didier.verkindt
F.~Vetrano,$^{121,122}$ %flavio.vetrano
A.~Vicer\'e,$^{121,122}$ %andrea.vicere
A.~D.~Viets,$^{21}$  %aaron.viets
S.~Vinciguerra,$^{58}$  %serena.vinciguerra
D.~J.~Vine,$^{27}$  %david.vine
J.-Y.~Vinet,$^{66}$ %jeanyves.vinet
S.~Vitale,$^{15}$ 	%salvatore.vitale
T.~Vo,$^{44}$  %thomas.vo
H.~Vocca,$^{42,43}$ %helios.vocca
C.~Vorvick,$^{47}$  %cheryl.vorvick
S.~P.~Vyatchanin,$^{61}$  %sergey.vyatchanin
A.~R.~Wade,$^{1}$  %andrew.wade
L.~E.~Wade,$^{84}$  %leslie.wade
M.~Wade,$^{84}$  %madeline.wade
R.~Walet,$^{14}$ %rob.walet
M.~Walker,$^{29}$  %marissa.walker
L.~Wallace,$^{1}$  %larry.wallace
S.~Walsh,$^{38,10,21}$  %sinead.walsh
G.~Wang,$^{17,122}$ %gang.wang
H.~Wang,$^{58}$  %haoyu.wang
J.~Z.~Wang,$^{63}$  %jonathan.wang
W.~H.~Wang,$^{102}$  %wenhui.wang
Y.~F.~Wang,$^{92}$  %yifan.wang
R.~L.~Ward,$^{25}$  %robert.ward
J.~Warner,$^{47}$  %jim.warner
M.~Was,$^{8}$ %michal.was
J.~Watchi,$^{97}$  %jennifer.watchi
B.~Weaver,$^{47}$  %betsy.weaver
L.-W.~Wei,$^{10,22}$  %li-wei.wei
M.~Weinert,$^{10}$  %michael.weinert
A.~J.~Weinstein,$^{1}$  %alan.weinstein
R.~Weiss,$^{15}$  %rainer.weiss
L.~Wen,$^{64}$  %linqing.wen
E.~K.~Wessel,$^{12}$  %erik.wessel
P.~We{\ss}els,$^{10}$  %peter.wessels
J.~Westerweck,$^{10}$  %julian.westerweck
T.~Westphal,$^{10}$  %tobias.westphal
K.~Wette,$^{25}$  %karl.wette
J.~T.~Whelan,$^{57}$  %john.whelan
B.~F.~Whiting,$^{5}$  %bernard.whiting
C.~Whittle,$^{6}$  %chris.whittle
D.~Wilken,$^{10}$  %dennis.schroeter
D.~Williams,$^{46}$  %daniel.williams
R.~D.~Williams,$^{1}$  %roy.williams
A.~R.~Williamson,$^{65}$  %andrew.williamson
J.~L.~Willis,$^{1,160}$  %joshua.willis
B.~Willke,$^{22,10}$  %benno.willke
M.~H.~Wimmer,$^{10}$  %maximilian.wimmer
W.~Winkler,$^{10}$  %walter.winkler
C.~C.~Wipf,$^{1}$  %christopher.wipf
H.~Wittel,$^{10,22}$  %holger.wittel
G.~Woan,$^{46}$  %graham.woan
J.~Woehler,$^{10}$  %janis.woehler
J.~Wofford,$^{57}$  %jared.wofford
K.~W.~K.~Wong,$^{92}$  %wang-kei.wong
J.~Worden,$^{47}$  %john.worden
J.~L.~Wright,$^{46}$  %jennifer.wright
D.~S.~Wu,$^{10}$  %david.wu
D.~M.~Wysocki,$^{57}$	%daniel.wysocki
S.~Xiao,$^{1}$  %sophia.xiao
H.~Yamamoto,$^{1}$  %hiro.yamamoto
C.~C.~Yancey,$^{75}$  %cregg.yancey
L.~Yang,$^{161}$  %le.yang
M.~J.~Yap,$^{25}$  %min-jet.yap
M.~Yazback,$^{5}$  %maher.yazback
Hang~Yu,$^{15}$  %hang.yu
Haocun~Yu,$^{15}$  %haocun.yu
M.~Yvert,$^{8}$ %michel.yvert
A.~Zadro\.zny,$^{132}$ %adam.zadrozny
M.~Zanolin,$^{37}$  %michele.zanolin
T.~Zelenova,$^{30}$ %tatiana.zelenova
J.-P.~Zendri,$^{54}$ %jean-pierre.zendri
M.~Zevin,$^{89}$  %michael.zevin
L.~Zhang,$^{1}$  %liyuan.zhang
M.~Zhang,$^{140}$  %mi.zhang
T.~Zhang,$^{46}$  %teng.zhang
Y.-H.~Zhang,$^{57}$  %yuanhao.zhang
C.~Zhao,$^{64}$  %chunnong.zhao
M.~Zhou,$^{89}$  %minchuan.zhou
Z.~Zhou,$^{89}$  %zifan.zhou
S.~J.~Zhu,$^{38,10}$  %sylvia.zhu
X.~J.~Zhu,$^{6}$ 	%xingjiang.zhu
M.~E.~Zucker,$^{1,15}$  %michael.zucker
and
J.~Zweizig$^{1}$%
\\
\medskip
(LIGO Scientific Collaboration and Virgo Collaboration) 
\\
\medskip
{${}^{\dag}$Deceased, February 2017. }% 
{${}^{\ddag}$Deceased, December 2016. }%  
}\noaffiliation
\affiliation {LIGO, California Institute of Technology, Pasadena, CA 91125, USA }% {CIT} {1}
\affiliation {Louisiana State University, Baton Rouge, LA 70803, USA }% {LSU} {2}
\affiliation {Universit\`a di Salerno, Fisciano, I-84084 Salerno, Italy }% {UNISA} {3}
\affiliation {INFN, Sezione di Napoli, Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy }% {INFN-NA} {4}
\affiliation {University of Florida, Gainesville, FL 32611, USA }% {UFlorida} {5}
\affiliation {OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia }% {MonashU} {6}
\affiliation {LIGO Livingston Observatory, Livingston, LA 70754, USA }% {LLO} {7}
\affiliation {Laboratoire d'Annecy-le-Vieux de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France }% {LAPP} {8}
\affiliation {University of Sannio at Benevento, I-82100 Benevento, Italy and INFN, Sezione di Napoli, I-80100 Napoli, Italy }% {USannio} {9}
\affiliation {Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany }% {AEIHannoverInst} {10}
\affiliation {The University of Mississippi, University, MS 38677, USA }% {UMiss} {11}
\affiliation {NCSA, University of Illinois at Urbana-Champaign, Urbana, IL 61801, USA }% {NCSARG} {12}
\affiliation {University of Cambridge, Cambridge CB2 1TN, United Kingdom }% {Cambridge} {13}
\affiliation {Nikhef, Science Park, 1098 XG Amsterdam, The Netherlands }% {NIKHEF} {14}
\affiliation {LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA }% {MIT} {15}
\affiliation {Instituto Nacional de Pesquisas Espaciais, 12227-010 S\~{a}o Jos\'{e} dos Campos, S\~{a}o Paulo, Brazil }% {GWINPE} {16}
\affiliation {Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy }% {GSSI} {17}
\affiliation {INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy }% {INFN-LNGS} {18}
\affiliation {Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India }% {IUCAA} {19}
\affiliation {International Centre for Theoretical Sciences, Tata Institute of Fundamental Research, Bengaluru 560089, India }% {ICTS-TIFR} {20}
\affiliation {University of Wisconsin-Milwaukee, Milwaukee, WI 53201, USA }% {UWM} {21}
\affiliation {Leibniz Universit\"at Hannover, D-30167 Hannover, Germany }% {Leibniz} {22}
\affiliation {Universit\`a di Pisa, I-56127 Pisa, Italy }% {UNIPI} {23}
\affiliation {INFN, Sezione di Pisa, I-56127 Pisa, Italy }% {INFN-PI} {24}
\affiliation {OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia }% {ANU} {25}
\affiliation {Laboratoire des Mat\'eriaux Avanc\'es (LMA), CNRS/IN2P3, F-69622 Villeurbanne, France }% {LMA} {26}
\affiliation {SUPA, University of the West of Scotland, Paisley PA1 2BE, United Kingdom }% {UWS} {27}
\affiliation {LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, F-91898 Orsay, France }% {LAL} {28}
\affiliation {California State University Fullerton, Fullerton, CA 92831, USA }% {Fullerton} {29}
\affiliation {European Gravitational Observatory (EGO), I-56021 Cascina, Pisa, Italy }% {EGO} {30}
\affiliation {Chennai Mathematical Institute, Chennai 603103, India }% {CMI} {31}
\affiliation {Universit\`a di Roma Tor Vergata, I-00133 Roma, Italy }% {UNITOV} {32}
\affiliation {INFN, Sezione di Roma Tor Vergata, I-00133 Roma, Italy }% {INFN-TOV} {33}
\affiliation {Universit\"at Hamburg, D-22761 Hamburg, Germany }% {ILP-UH} {34}
\affiliation {INFN, Sezione di Roma, I-00185 Roma, Italy }% {INFN-RM1} {35}
\affiliation {Cardiff University, Cardiff CF24 3AA, United Kingdom }% {Cardiff} {36}
\affiliation {Embry-Riddle Aeronautical University, Prescott, AZ 86301, USA }% {EmbryRiddle} {37}
\affiliation {Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-14476 Potsdam-Golm, Germany }% {AEIGolm} {38}
\affiliation {APC, AstroParticule et Cosmologie, Universit\'e Paris Diderot, CNRS/IN2P3, CEA/Irfu, Observatoire de Paris, Sorbonne Paris Cit\'e, F-75205 Paris Cedex 13, France }% {APC} {39}
\affiliation {Korea Institute of Science and Technology Information, Daejeon 34141, Korea }% {KISTI} {40}
\affiliation {West Virginia University, Morgantown, WV 26506, USA }% {WVU} {41}
\affiliation {Universit\`a di Perugia, I-06123 Perugia, Italy }% {UNIPG} {42}
\affiliation {INFN, Sezione di Perugia, I-06123 Perugia, Italy }% {INFN-PG} {43}
\affiliation {Syracuse University, Syracuse, NY 13244, USA }% {Syracuse} {44}
\affiliation {University of Minnesota, Minneapolis, MN 55455, USA }% {UMinnesota} {45}
\affiliation {SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom }% {Glasgow} {46}
\affiliation {LIGO Hanford Observatory, Richland, WA 99352, USA }% {LHO} {47}
\affiliation {Caltech CaRT, Pasadena, CA 91125, USA }% {CaRT} {48}
\affiliation {Wigner RCP, RMKI, H-1121 Budapest, Konkoly Thege Mikl\'os \'ut 29-33, Hungary }% {RMKI} {49}
\affiliation {Columbia University, New York, NY 10027, USA }% {Columbia} {50}
\affiliation {Stanford University, Stanford, CA 94305, USA }% {Stanford} {51}
\affiliation {Universit\`a di Camerino, Dipartimento di Fisica, I-62032 Camerino, Italy }% {UNICAM} {52}
\affiliation {Universit\`a di Padova, Dipartimento di Fisica e Astronomia, I-35131 Padova, Italy }% {UNIPD} {53}
\affiliation {INFN, Sezione di Padova, I-35131 Padova, Italy }% {INFN-PD} {54}
\affiliation {Institute of Physics, E\"otv\"os University, P\'azm\'any P. s. 1/A, Budapest 1117, Hungary }% {Eotvos} {55}
\affiliation {Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716, Warsaw, Poland }% {CAMK} {56}
\affiliation {Rochester Institute of Technology, Rochester, NY 14623, USA }% {RIT} {57}
\affiliation {University of Birmingham, Birmingham B15 2TT, United Kingdom }% {Birmingham} {58}
\affiliation {INFN, Sezione di Genova, I-16146 Genova, Italy }% {INFN-GE} {59}
\affiliation {RRCAT, Indore MP 452013, India }% {RRCAT} {60}
\affiliation {Faculty of Physics, Lomonosov Moscow State University, Moscow 119991, Russia }% {MoscowState} {61}
\affiliation {SUPA, University of Strathclyde, Glasgow G1 1XQ, United Kingdom }% {Strathclyde} {62}
\affiliation {The Pennsylvania State University, University Park, PA 16802, USA }% {PennState} {63}
\affiliation {OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia }% {UWesternAustralia} {64}
\affiliation {Department of Astrophysics/IMAPP, Radboud University Nijmegen, P.O. Box 9010, 6500 GL Nijmegen, The Netherlands }% {UNIRAD} {65}
\affiliation {Artemis, Universit\'e C\^ote d'Azur, Observatoire C\^ote d'Azur, CNRS, CS 34229, F-06304 Nice Cedex 4, France }% {ARTEMIS} {66}
\affiliation {Institut FOTON, CNRS, Universit\'e de Rennes 1, F-35042 Rennes, France }% {UNIRENN} {67}
\affiliation {Washington State University, Pullman, WA 99164, USA }% {WashingtonState} {68}
\affiliation {University of Oregon, Eugene, OR 97403, USA }% {UOregon} {69}
\affiliation {Laboratoire Kastler Brossel, UPMC-Sorbonne Universit\'es, CNRS, ENS-PSL Research University, Coll\`ege de France, F-75005 Paris, France }% {LKB} {70}
\affiliation {Carleton College, Northfield, MN 55057, USA }% {Carleton} {71}
\affiliation {OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia }% {UAdelaide} {72}
\affiliation {Astronomical Observatory Warsaw University, 00-478 Warsaw, Poland }% {ASTRO-W} {73}
\affiliation {VU University Amsterdam, 1081 HV Amsterdam, The Netherlands }% {UNIAMST} {74}
\affiliation {University of Maryland, College Park, MD 20742, USA }% {UMaryland} {75}
\affiliation {Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA }% {GaTech} {76}
\affiliation {Universit\'e Claude Bernard Lyon 1, F-69622 Villeurbanne, France }% {UNILYON1} {77}
\affiliation {Universit\`a di Napoli `Federico II,' Complesso Universitario di Monte S.Angelo, I-80126 Napoli, Italy }% {UNINA} {78}
\affiliation {NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA }% {Goddard} {79}
\affiliation {Dipartimento di Fisica, Universit\`a degli Studi di Genova, I-16146 Genova, Italy }% {UNIGE} {80}
\affiliation {RESCEU, University of Tokyo, Tokyo, 113-0033, Japan. }% {UTokyo} {81}
\affiliation {Tsinghua University, Beijing 100084, China }% {Tsinghua} {82}
\affiliation {Texas Tech University, Lubbock, TX 79409, USA }% {TTU} {83}
\affiliation {Kenyon College, Gambier, OH 43022, USA }% {Kenyon} {84}
\affiliation {Departamento de Astronom\'{\i }a y Astrof\'{\i }sica, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain }% {ASTROVAL} {85}
\affiliation {Museo Storico della Fisica e Centro Studi e Ricerche Enrico Fermi, I-00184 Roma, Italy }% {FERMI} {86}
\affiliation {National Tsing Hua University, Hsinchu City, 30013 Taiwan, Republic of China }% {NTHU} {87}
\affiliation {Charles Sturt University, Wagga Wagga, New South Wales 2678, Australia }% {CharlesSturt} {88}
\affiliation {Center for Interdisciplinary Exploration \& Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA }% {Northwestern} {89}
\affiliation {University of Chicago, Chicago, IL 60637, USA }% {UChicago} {90}
\affiliation {Pusan National University, Busan 46241, Korea }% {PusanNationalU} {91}
\affiliation {The Chinese University of Hong Kong, Shatin, NT, Hong Kong }% {CUHK} {92}
\affiliation {INAF, Osservatorio Astronomico di Padova, I-35122 Padova, Italy }% {INAF-PD} {93}
\affiliation {INFN, Trento Institute for Fundamental Physics and Applications, I-38123 Povo, Trento, Italy }% {INFN-TIFPA} {94}
\affiliation {OzGrav, University of Melbourne, Parkville, Victoria 3010, Australia }% {UMelbourne} {95}
\affiliation {Universit\`a di Roma `La Sapienza,' I-00185 Roma, Italy }% {UNIRM1} {96}
\affiliation {Universit\'e Libre de Bruxelles, Brussels 1050, Belgium }% {ULB} {97}
\affiliation {Sonoma State University, Rohnert Park, CA 94928, USA }% {SonomaState} {98}
\affiliation {Departamento de Matem\'aticas, Universitat de Val\`encia, E-46100 Burjassot, Val\`encia, Spain }% {MATEVAL} {99}
\affiliation {Montana State University, Bozeman, MT 59717, USA }% {MontanaState} {100}
\affiliation {Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain }% {BalearicIslands} {101}
\affiliation {The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA }% {CGWA-UTRGV} {102}
\affiliation {Bellevue College, Bellevue, WA 98007, USA }% {BC} {103}
\affiliation {Institute for Plasma Research, Bhat, Gandhinagar 382428, India }% {IPR-Bhat} {104}
\affiliation {The University of Sheffield, Sheffield S10 2TN, United Kingdom }% {USheffield} {105}
\affiliation {Dipartimento di Scienze Matematiche, Fisiche e Informatiche, Universit\`a di Parma, I-43124 Parma, Italy }% {UNIPR} {106}
\affiliation {INFN, Sezione di Milano Bicocca, Gruppo Collegato di Parma, I-43124 Parma, Italy }% {INFN-PR} {107}
\affiliation {California State University, Los Angeles, 5151 State University Dr, Los Angeles, CA 90032, USA }% {CalStateLA} {108}
\affiliation {Universit\`a di Trento, Dipartimento di Fisica, I-38123 Povo, Trento, Italy }% {UNITN} {109}
\affiliation {Montclair State University, Montclair, NJ 07043, USA }% {MontclairState} {110}
\affiliation {National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan }% {NAOJ} {111}
\affiliation {Canadian Institute for Theoretical Astrophysics, University of Toronto, Toronto, Ontario M5S 3H8, Canada }% {CITA} {112}
\affiliation {Observatori Astron\`omic, Universitat de Val\`encia, E-46980 Paterna, Val\`encia, Spain }% {OAVAL} {113}
\affiliation {School of Mathematics, University of Edinburgh, Edinburgh EH9 3FD, United Kingdom }% {Edinburgh} {114}
\affiliation {University and Institute of Advanced Research, Koba Institutional Area, Gandhinagar Gujarat 382007, India }% {UIAS} {115}
\affiliation {IISER-TVM, CET Campus, Trivandrum Kerala 695016, India }% {IISER-TVM} {116}
\affiliation {University of Szeged, D\'om t\'er 9, Szeged 6720, Hungary }% {SZTE} {117}
\affiliation {University of Michigan, Ann Arbor, MI 48109, USA }% {UMichigan} {118}
\affiliation {Tata Institute of Fundamental Research, Mumbai 400005, India }% {TIFR} {119}
\affiliation {INAF, Osservatorio Astronomico di Capodimonte, I-80131, Napoli, Italy }% {INAF-NA} {120}
\affiliation {Universit\`a degli Studi di Urbino `Carlo Bo,' I-61029 Urbino, Italy }% {UNIURB} {121}
\affiliation {INFN, Sezione di Firenze, I-50019 Sesto Fiorentino, Firenze, Italy }% {INFN-FI} {122}
\affiliation {Physik-Institut, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland }% {UZH} {123}
\affiliation {American University, Washington, D.C. 20016, USA }% {American} {124}
\affiliation {University of Bia{\l }ystok, 15-424 Bia{\l }ystok, Poland }% {UNIBIALI} {125}
\affiliation {University of Southampton, Southampton SO17 1BJ, United Kingdom }% {Southampton} {126}
\affiliation {University of Washington Bothell, 18115 Campus Way NE, Bothell, WA 98011, USA }% {Bothell} {127}
\affiliation {Institute of Applied Physics, Nizhny Novgorod, 603950, Russia }% {NizhnyNovgorod} {128}
\affiliation {Korea Astronomy and Space Science Institute, Daejeon 34055, Korea }% {KASI} {129}
\affiliation {Inje University Gimhae, South Gyeongsang 50834, Korea }% {InjeU} {130}
\affiliation {National Institute for Mathematical Sciences, Daejeon 34047, Korea }% {NIMS} {131}
\affiliation {NCBJ, 05-400 \'Swierk-Otwock, Poland }% {NCBJ} {132}
\affiliation {Institute of Mathematics, Polish Academy of Sciences, 00656 Warsaw, Poland }% {IMPAN} {133}
\affiliation {Hillsdale College, Hillsdale, MI 49242, USA }% {Hillsdale} {134}
\affiliation {Hanyang University, Seoul 04763, Korea }% {HanyangU} {135}
\affiliation {Seoul National University, Seoul 08826, Korea }% {SeoulNationalU} {136}
\affiliation {NASA Marshall Space Flight Center, Huntsville, AL 35811, USA }% {NASA-MSFC} {137}
\affiliation {ESPCI, CNRS, F-75005 Paris, France }% {ESPCI} {138}
\affiliation {Southern University and A\&M College, Baton Rouge, LA 70813, USA }% {SouthernU} {139}
\affiliation {College of William and Mary, Williamsburg, VA 23187, USA }% {CWM} {140}
\affiliation {Centre Scientifique de Monaco, 8 quai Antoine Ier, MC-98000, Monaco }% {CSMON} {141}
\affiliation {Indian Institute of Technology Madras, Chennai 600036, India }% {IIT-Madras} {142}
\affiliation {IISER-Kolkata, Mohanpur, West Bengal 741252, India }% {IISER-KOL} {143}
\affiliation {Whitman College, 345 Boyer Avenue, Walla Walla, WA 99362 USA }% {Whitman} {144}
\affiliation {Indian Institute of Technology Bombay, Powai, Mumbai, Maharashtra 400076, India }% {Bombay} {145}
\affiliation {Scuola Normale Superiore, Piazza dei Cavalieri 7, I-56126 Pisa, Italy }% {SNS} {146}
\affiliation {Universit\'e de Lyon, F-69361 Lyon, France }% {UNILYON} {147}
\affiliation {Hobart and William Smith Colleges, Geneva, NY 14456, USA }% {HobartWilliamSmith} {148}
\affiliation {OzGrav, Swinburne University of Technology, Hawthorn VIC 3122, Australia }% {Swinburne} {149}
\affiliation {Janusz Gil Institute of Astronomy, University of Zielona G\'ora, 65-265 Zielona G\'ora, Poland }% {ASTRO-Z} {150}
\affiliation {University of Washington, Seattle, WA 98195, USA }% {UWashGravity} {151}
\affiliation {King's College London, University of London, London WC2R 2LS, United Kingdom }% {KCL} {152}
\affiliation {Indian Institute of Technology, Gandhinagar Ahmedabad Gujarat 382424, India }% {IITGN} {153}
\affiliation {Indian Institute of Technology Hyderabad, Sangareddy, Khandi, Telangana 502285, India }% {IIT-Hydera} {154}
\affiliation {International Institute of Physics, Universidade Federal do Rio Grande do Norte, Natal RN 59078-970, Brazil }% {IIP-UFRN} {155}
\affiliation {Andrews University, Berrien Springs, MI 49104, USA }% {Andrews} {156}
\affiliation {Universit\`a di Siena, I-53100 Siena, Italy }% {UNISI} {157}
\affiliation {Trinity University, San Antonio, TX 78212, USA }% {Trinity} {158}
\affiliation {Van Swinderen Institute for Particle Physics and Gravity, University of Groningen, Nijenborgh 4, 9747 AG Groningen, The Netherlands }% {UNIGRON} {159}
\affiliation {Abilene Christian University, Abilene, TX 79699, USA }% {ACU} {160}
\affiliation {Colorado State University, Fort Collins, CO 80523, USA }% {CSU} {161}

%\date[\relax]{Dated: 10/5/2017}
%\maketitle
%\end{document}


==> GW170817_ Implications for the Stochastic Gravitational-Wave Background from Compact Binary Coalescences/LVCack.tex <==
The authors gratefully acknowledge the support of the United States
National Science Foundation (NSF) for the construction and operation of the
LIGO Laboratory and Advanced LIGO as well as the Science and Technology Facilities Council (STFC) of the
United Kingdom, the Max-Planck-Society (MPS), and the State of
Niedersachsen/Germany for support of the construction of Advanced LIGO 
and construction and operation of the GEO600 detector. 
Additional support for Advanced LIGO was provided by the Australian Research Council.
The authors gratefully acknowledge the Italian Istituto Nazionale di Fisica Nucleare (INFN),  
the French Centre National de la Recherche Scientifique (CNRS) and
the Foundation for Fundamental Research on Matter supported by the Netherlands Organisation for Scientific Research, 
for the construction and operation of the Virgo detector
and the creation and support  of the EGO consortium. 
The authors also gratefully acknowledge research support from these agencies as well as by 
the Council of Scientific and Industrial Research of India, 
the Department of Science and Technology, India,
the Science \& Engineering Research Board (SERB), India,
the Ministry of Human Resource Development, India,
the Spanish  Agencia Estatal de Investigaci\'on,
the  Vicepresid\`encia i Conselleria d'Innovaci\'o, Recerca i Turisme and the Conselleria d'Educaci\'o i Universitat del Govern de les Illes Balears,
the Conselleria d'Educaci\'o, Investigaci\'o, Cultura i Esport de la Generalitat Valenciana,
the National Science Centre of Poland,
the Swiss National Science Foundation (SNSF),
the Russian Foundation for Basic Research, 
the Russian Science Foundation,
the European Commission,
the European Regional Development Funds (ERDF),
the Royal Society, 
the Scottish Funding Council, 
the Scottish Universities Physics Alliance, 
the Hungarian Scientific Research Fund (OTKA),
the Lyon Institute of Origins (LIO),
the National Research, Development and Innovation Office Hungary (NKFI), 
the National Research Foundation of Korea,
Industry Canada and the Province of Ontario through the Ministry of Economic Development and Innovation, 
the Natural Science and Engineering Research Council Canada,
the Canadian Institute for Advanced Research,
the Brazilian Ministry of Science, Technology, Innovations, and Communications,
the International Center for Theoretical Physics South American Institute for Fundamental Research (ICTP-SAIFR), 
the Research Grants Council of Hong Kong,
the National Natural Science Foundation of China (NSFC),
the Leverhulme Trust, 
the Research Corporation, 
the Ministry of Science and Technology (MOST), Taiwan
and
the Kavli Foundation.
The authors gratefully acknowledge the support of the NSF, STFC, MPS, INFN, CNRS and the
State of Niedersachsen/Germany for provision of computational resources.


==> GW170817_ Implications for the Stochastic Gravitational-Wave Background from Compact Binary Coalescences/implications_macros.tex <==
%BNS Rate
\def\bnsrate{1540^{+3200}_{-1220} \text{ Gpc}^{-3}\text{ yr}^{-1}}

% BBH Rate
\def\bbhrate{103^{+110}_{-63} \text{ Gpc}^{-3}\text{ yr}^{-1}}

% omega BNS
\def\OmegaBNSMean{0.7}
\newcommand{\OmegaRangeBNS}{\ensuremath{\OmegaBNSMean_{-0.6}^{+1.5} \times 10^{-9} }}

% omega BBH
\def\OmegaBBHMean{1.1}
\newcommand{\OmegaRangeBBH}
{\ensuremath{\OmegaBBHMean_{-0.7}^{+1.2} \times 10^{-9} }}

% omega Total
\def\OmegaTotMean{1.8}
\newcommand{\OmegaRange}{\ensuremath{\OmegaTotMean_{-1.3}^{+2.7} \times 10^{-9} }}

% tau
\newcommand{\tauBNS}{\ensuremath{13_{-9}^{+49} }}
\newcommand{\tauBBH}{\ensuremath{223_{-115}^{+352} }}
\newcommand{\tauTotal}{\ensuremath{12_{-8}^{44} }}

% lambda
\newcommand{\lambdaBNS}{\ensuremath{15 ^{+30} _{-12}}}
\newcommand{\lambdaBBH}{\ensuremath{0.06 ^{+0.06} _{-0.04}}}
\newcommand{\lambdaTot}{\ensuremath{15 ^{+31} _{-12}}}

% duration
\newcommand{\durBNS}{190}
\newcommand{\durBBH}{14}

% time to observation
\def\obs{40 months}
\def\obsopt{18 months}
\def\obsbound{40(18) months}


